Counterfactual Fair Opportunity: Measuring Decision Model Fairness with Counterfactual Reasoning

The increasing application of Artificial Intelligence and Machine Learning models poses potential risks of unfair behavior and, in light of recent regulations, has attracted the attention of the research community. Several researchers focused on seeking new fairness definitions or developing approaches to identify biased predictions. However, none try to exploit the counterfactual space to this aim. In that direction, the methodology proposed in this work aims to unveil unfair model behaviors using counterfactual reasoning in the case of fairness under unawareness setting. A counterfactual version of equal opportunity named counterfactual fair opportunity is defined and two novel metrics that analyze the sensitive information of counterfactual samples are introduced. Experimental results on three different datasets show the efficacy of our methodologies and our metrics, disclosing the unfair behavior of classic machine learning and debiasing models.

==> tables/newMetrics.tex <==
\begin{table*}[ht]
% \vspace{-2mm}
    \centering
    \scriptsize
    \caption{AUC, ACC, DSP, DEO, and DAO results on Test set; \text{CFlip} and \text{nDCG} results at different $|k|$ number of Counterfactuals for each negatively predicted Test set sample, ($0^*$ there are no negative predicted \textit{unprivileged} samples which result in no CF samples for the unprivileged group, hence SVM $\Delta$CFlip@10 denoted with the $\dagger$ cannot be considered as the best result).}
    \label{tab:totResCFLIPNDCCF}
    \begin{adjustbox}{width=\textwidth, center}
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1}
\rowcolors{12}{gray!15}{white}
\begin{tabular}{llrrrrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\toprule
& & & & & & \multicolumn{1}{c}{}  & \multicolumn{9}{c}{$\text{CFlips}$@$|k|$ (\%)} & \multicolumn{9}{c}{$\text{nDCCF}@|k|$}
\\ \cmidrule(lr){8-16} \cmidrule(lr){17-25}
& & &  & & &  \multicolumn{1}{c}{} & \multicolumn{3}{c}{Privileged} & \multicolumn{3}{c}{Unprivileged} & \multicolumn{3}{c}{$\Delta\text{CFlips}\downarrow
$}&\multicolumn{3}{c}{Privileged} & \multicolumn{3}{c}{Unprivileged} & \multicolumn{3}{c}{$\Delta\text{nDCCF}\downarrow
$} \\ \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22} \cmidrule(lr){23-25}  
 Dataset   & model    & AUC$\uparrow$ &  ACC$\uparrow$ &   DSP$\downarrow$ & DEO$\downarrow$
 &   \multicolumn{1}{c}{DAO$\downarrow$
} &   @10 &   @50 &   \multicolumn{1}{c}{@100} &   @10 &   @50 &   \multicolumn{1}{c}{@100} &   @10 &   @50 &   \multicolumn{1}{c}{@100} &   @10 & @50 & \multicolumn{1}{c}{@100} & @10 &   @50 &   \multicolumn{1}{c}{@100} & @10 & @50 &   @100 \\
 \hline
\midrule
     & LR      & 0.9078 &   0.8099 &     0.2947 &     0.1790 & 0.1474  &     12.332 &        10.886 &         10.212 &        66.353 &        72.932 &         77.165 &        54.021 &        62.046 &         66.953 &        0.8678 &        0.8849 &         0.886  &        0.3522 &        0.2913 &         0.2497 &               0.5156 &               0.5936 &                0.6363 \\
\cellcolor{white}   & SVM     & 0.9073 &    0.8541 &     0.1769 &     0.1297 & 0.0884   &     6.752 &         7.533 &          7.742 &        77.095 &        80.973 &         81.372 &        70.343 &        73.44  &         73.63  &        0.9306 &        0.9258 &         0.9171 &        0.2474 &        0.2042 &         0.1948 &               0.6832 &               0.7216 &                0.7223 \\
\cellcolor{white}   & LGB     & 0.9304  &  0.8658 &     0.1850 &     0.1368 &  0.0925  &     9.195 &         8.541 &          8.781 &        65.918 &        76.605 &         79.697 &        56.723 &        68.064 &         70.916 &        0.9049 &        0.9124 &         0.9049 &        0.3611 &        0.2633 &         0.2272 &               0.5438 &               0.6491 &                0.6777 \\
\cellcolor{white}   & XGB     & \textbf{0.9314}   &  \textbf{0.8698} &     0.1884 &     0.1425 &   0.0941  &   10.011 &         8.788 &          9.07  &        64.796 &        76.243 &         79.512 &        54.785 &        67.455 &         70.442 &        0.8968 &        0.9088 &         0.9014 &        0.3708 &        0.2677 &         0.2298 &               0.526  &               0.6411 &                0.6716 \\
\cellcolor{white}   & AdvDeb  & 0.9123 &  0.8512 &     \textbf{0.1150} &     \textbf{0.0992} &  \textbf{0.0575}   &   30.046 &        34.488 &         34.968 &        36.11  &        38.694 &         43.041 &         6.064 &         \textbf{4.206} &          \textbf{8.073} &        0.7016 &        0.6668 &         0.6537 &        0.6427 &        0.6199 &         0.5812 &               0.0589 &               \textbf{0.0469} &                \textbf{0.0725} \\
  \multirow{-6}{*}{\cellcolor{white}Adult}  & lferm   &  0.9031  & 0.8428 &     0.1448 &     0.1118 &   0.0724 &   31.459 &        28.632 &         24.965 &        31.764 &        47.464 &         57.47  &         \textbf{0.305} &        18.832 &         32.505 &        0.6857 &        0.7062 &         0.7314 &        0.6864 &        0.5632 &         0.4701 &               \textbf{0.0007} &               0.143  &                0.2613 \\
\midrule
    & LR      &  0.8233 &  0.7367 &     0.1567 &     0.1515 &  0.0783   &    8.438 &        10.838 &         13.192 &        54.816 &        57.521 &         57.047 &        46.378 &        46.683 &         43.855 &        0.9239 &        0.9012 &         0.8736 &        0.464  &        0.4332 &         0.4303 &               0.4599 &               0.468  &                0.4433 \\
   \cellcolor{white} & SVM     & 0.8189 &   0.7395 &     0.1062 &     0.1425 &    0.0894  &  11.937 &        16.377 &         17.379 &        31.305 &        33.869 &         35.385 &        \textbf{19.368} &        \textbf{17.492} &         \textbf{18.006} &        0.8871 &        0.8468 &         0.8295 &        0.6661 &        0.6616 &         0.6449 &               \textbf{0.221}  &               \textbf{0.1852} &                \textbf{0.1846}\\
  \cellcolor{white}  & LGB     & \textbf{0.8596}  &  0.8371 &     0.1093 &     0.0968 &  0.0546   &    4.596 &         9.384 &         12.817 &        66.779 &        74.088 &         73.366 &        62.183 &        64.704 &         60.549 &        0.958  &        0.9185 &         0.8818 &        0.3744 &        0.2879 &         0.2804 &               0.5836 &               0.6306 &                0.6014 \\
  \cellcolor{white}  & XGB     & 0.8578  &  \textbf{0.8375} &     0.1056 &     0.0958 &   0.0528  &    1.803 &         3.152 &          6.523 &        81.289 &        88.9   &         84.48  &        79.486 &        85.748 &         77.957 &        0.9804 &        0.9711 &         0.9386 &        0.2183 &        0.1378 &         0.1599 &               0.7621 &               0.8333 &                0.7787 \\
   \cellcolor{white} & AdvDeb  & 0.8309  &  0.8195 &     0.0957 &     0.0852 &  0.0479   &   16.369 &        20.067 &         23.123 &        44.722 &        52.645 &         57.043 &        28.353 &        32.578 &         33.92  &        0.8493 &        0.8119 &         0.7787 &        0.5803 &        0.4998 &         0.4536 &               0.269  &               0.3121 &                0.3251 \\
 \multirow{-6}{*}{\cellcolor{white}AdultDeb}   & lferm   & 0.8017   & 0.7953 &     \textbf{0.0639} &     \textbf{0.0563} &    \textbf{0.0320}   &  8.943 &        13.316 &         16.561 &        47.036 &        54.87  &         55.83  &        38.093 &        41.554 &         39.269 &        0.9248 &        0.8809 &         0.8452 &        0.5618 &        0.4791 &         0.4584 &               0.363  &               0.4018 &                0.3868 \\

\midrule
     & LR      & 0.9248  &  \textbf{0.8700} &     0.6535 &     0.5738 &  0.3267  &     2.857 &         3.429 &          3.667 &        75.286 &        81.943 &         85.143 &        72.429 &        78.514 &         81.476 &        0.9688 &        0.9656 &         0.9568 &        0.2659 &        0.2011 &         0.1678 &               0.7029 &               0.7645 &                0.789  \\
  \cellcolor{white}  & SVM     & \textbf{0.9288}  &  \textbf{0.8700} &     0.6395 &     0.5772 &  0.3198  &     6.25  &         5.917 &          5.63  &        73.239 &        80.789 &         84.493 &        66.989 &        74.872 &         78.863 &        0.938  &        0.94   &         0.9359 &        0.2868 &        0.2149 &         0.1776 &               0.6512 &               0.7251 &                0.7583 \\
    \cellcolor{white}& LGB     & 0.9168  &  0.8400 &     0.6363 &     0.5394 &  0.3181  &     5.652 &         5.913 &          5.696 &        74.571 &        80.143 &         83.55  &        68.919 &        74.23  &         77.854 &        0.9424 &        0.9407 &         0.9357 &        0.2875 &        0.2215 &         0.1854 &               0.6549 &               0.7192 &                0.7503 \\
 \cellcolor{white}   & XGB     & 0.9099  &  0.8500 &     0.6568 &     0.5480 &   0.3284   &   5     &         5.455 &          5.045 &        73.38  &        80.141 &         83.613 &        68.38  &        74.686 &         78.568 &        0.9492 &        0.9467 &         0.9427 &        0.2938 &        0.2214 &         0.1851 &               0.6554 &               0.7253 &                0.7576 \\
   & AdvDeb  &  0.9008 &  0.8100 &     \textbf{0.5501} &     \textbf{0.4704} &  \textbf{0.2750}   &    7.576 &         7.03  &          7.273 &        69     &        77.571 &         80.643 &        61.424 &        70.541 &         73.37  &        0.9295 &        0.9295 &         0.9209 &        0.3396 &        0.2519 &         0.2164 &               0.5899 &               0.6776 &                0.7045 \\
 \multirow{-6}{*}{\cellcolor{white} Crime}  & lferm   & 0.9100   & 0.8400 &     0.6125 &     0.5480 &   0.3062   &   3.913 &         6.174 &          6.696 &        64.412 &        71.588 &         75.103 &        \textbf{60.499} &        \textbf{65.414} &         \textbf{68.407} &        0.9592 &        0.9408 &         0.929  &        0.3695 &        0.305  &         0.2686 &               \textbf{0.5897} &               \textbf{0.6358} &                \textbf{0.6604} \\
\midrule
   & LR      & \textbf{0.8186}  &  0.7600 &     0.1187 &     \textbf{0.0299} &  0.0593  &     4.4   &         6.56  &          7.402 & 30.000        & 28.000        & 34.000         &        25.6   &        21.44  &         26.598 &        0.9656 &        0.9417 &         0.9267 & 0.7289        & 0.7197        & 0.6728         &               0.2367 &               0.222  &                0.2539 \\
\cellcolor{white}    & SVM     &  0.8109 &  0.7600 &     0.0449 &     0.0538 &  0.0762   &    6.667 &         9.167 &         10     &$0^*$           &$0^*$           &$0^*$            &         $\mathbf{6.667^\dagger}$ &         9.167 &         10     &        0.9276 &        0.9124 &         0.8985 &$0^*$           &$0^*$           &$0^*$            &               0.9276 &               0.9124 &                0.8985 \\
   & LGB     &  0.7614  & 0.7500 &     0.1632 &     0.1973 &   0.1157   &  10     &        11.833 &         13.833 & 30.000        & 42.000        & 47.000         &        20     &        30.167 &         33.167 &        0.8912 &        0.8836 &         0.8608 & 0.6643        & 0.5901        & 0.5462         &               0.2269 &               0.2935 &                0.3146 \\
 \cellcolor{white}   & XGB     &  0.7871  & \textbf{0.7900} &     0.0518 &     0.1005 &   0.0746   &  12.727 &        13.091 &         14     & 0.000         & 12.000        & 20.500         &        \textbf{12.727} &         \textbf{1.091} &          \textbf{6.5}   &        0.8755 &        0.8713 &         0.8573 & 1.0000        & 0.9040        & 0.8268         &               \textbf{0.1245} &               \textbf{0.0327} &                \textbf{0.0305} \\
   & AdvDeb  &  0.7371  & 0.7300 &     0.1809 &     0.2150 &  0.1246     &  4.545 &         7.455 &         10.364 & 40.000        & 60.000        & 66.000         &        35.455 &        52.545 &         55.636 &        0.959  &        0.9336 &         0.9015 & 0.6619        & 0.4579        & 0.3906         &               0.2971 &               0.4757 &                0.5109 \\
 \multirow{-6}{*}{\cellcolor{white}German}   & lferm   &  0.7605  & 0.7200 &     \textbf{0.0355} &     0.0650 &   \textbf{0.0472}   &  15     &         8     &         12.5   &$0^*$           &$0^*$           &$0^*$            &        15     &         8     &         12.5   &        0.8002 &        0.8863 &         0.8572 &$0^*$           &$0^*$           &$0^*$            &               0.8002 &               0.8863 &                0.8572 \\
\hline
\bottomrule
\hline
\end{tabular}
\end{adjustbox}
\vspace{-4mm}
\end{table*}
